RefinedFields: Radiance Fields Refinement for Planar Scene Representations

Planar scene representations have recently witnessed increased interests for modeling scenes from images, as their lightweight planar structure enables compatibility with image-based models. Notably, K-Planes have gained particular attention as they extend planar scene representations to support in-the-wild scenes, in addition to object-level scenes. However, their visual quality has recently lagged behind that of state-of-the-art techniques. To reduce this gap, we propose RefinedFields, a method that leverages pre-trained networks to refine K-Planes scene representations via optimization guidance using an alternating training procedure. We carry out extensive experiments and verify the merit of our method on synthetic data and real tourism photo collections. RefinedFields enhances rendered scenes with richer details and improves upon its base representation on the task of novel view synthesis. Our project page can be found at https://refinedfields.github.io .

==> tables/training-times.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Training times.} Comparison of training time among methods tackling novel view synthesis in-the-wild. Timings are based on a single NVIDIA V100 GPU. Our method improves upon K-Planes while still requiring significantly less training time than other works.\\
$^{*}$ Methods trained in a half-resolution setting.}
\vskip 0.15in
{\footnotesize
\begin{tabular}{l c} \toprule
     & Training Time ($\downarrow$)\\ \midrule
    NeRF-W \citep{nerf-w} & 400 hrs \\
    $\text{Ha-NeRF}^{*}$ \citep{ha-nerf} & 452 hrs \\
    $\text{CR-NeRF}^{*}$ \citep{cr-nerf} & 420 hrs \\
    K-Planes \citep{kplanes} & 50 mins \\ \midrule
    RefinedFields (ours) & 150 hrs \\ \bottomrule
\end{tabular}
}
\label{table:training-times}
\end{table}

